Cooperative Multi-agent Bandits: Distributed Algorithms with Optimal Individual Regret and Constant Communication Costs

Recently, there has been extensive study of cooperative multi-agent multi-armed bandits where a set of distributed agents cooperatively play the same multi-armed bandit game. The goal is to develop bandit algorithms with the optimal group and individual regrets and low communication between agents. The prior work tackled this problem using two paradigms: leader-follower and fully distributed algorithms. Prior algorithms in both paradigms achieve the optimal group regret. The leader-follower algorithms achieve constant communication costs but fail to achieve optimal individual regrets. The state-of-the-art fully distributed algorithms achieve optimal individual regrets but fail to achieve constant communication costs. This paper presents a simple yet effective communication policy and integrates it into a learning algorithm for cooperative bandits. Our algorithm achieves the best of both paradigms: optimal individual regret and constant communication costs.

==> doe_ucb.tex <==
\section{UCB Design}

In this section, we try to devise a UCB-type \alg algorithm with constant communications and near-optimal group and individual regrets.

\begin{algorithm}[H]
    \caption{The Bandit Learning Algorithm for Agent $j$ (UCB) }
    \label{alg:3}
    \footnotesize
    \begin{algorithmic}[1]
        \State \textbf{Parameters:} \(\alpha > 0\) and \(\beta > 1\)
        \State \textbf{Initialization:} $\hat{\mu}_{\texttt{com}}(i), n_t^j(i) \leftarrow 0$, $\hat{\mu}^j_{\texttt{aux},t}(i),\hat{\mu}_t^j(i), \ei_{\tau(t)}^j(i)\gets \infty$, for all $i$, and $g(n)\leftarrow \alpha \ci(Mn,\delta)$, $n=1,2,\ldots$
        \For{each round $t$}

        \State Pull an arm $i\gets \arg\max_{i'} \hat{\mu}_t^j(i') + \ci(Mn_t^j(i'),\delta)$


        \If {$\beta g(n_t^j(i))\leq\ei_{\tau(t)}^j(i)$}
        \State $\ei_{\tau(t)}^j(i)\leftarrow g(n_t^j(i))$

        \If {$|\hat{\mu}_{\texttt{aux},t}^j(i)-\hat{\mu}_{\texttt{com}}(i)|>g(n_t^j(i))$}
        \State{\texttt{//Communicate to synchronize the estimates}}
        \State{--- Collect $X_t^{j'}(i)$ from other agents \(j'\neq j\) and calculate the new $\hat{\mu}_{\texttt{com}}(i)$}
        \State --- Broadcast the new $\hat{\mu}_{\texttt{com}}(i)$ to other agents \(j'\neq j\)
        \State --- $X_{\tau(t)}^{j'}(i)\leftarrow X_t^{j'}(i)$ for all $j'\in \mathcal{M}$
        \EndIf
        \EndIf

        \State Update $n_{t+1}^j(i), \hat{\mu}_{t+1}^j(i)$, and $\hat{\mu}_{\texttt{aux},t+1}^j(i)$
        \EndFor
    \end{algorithmic}
\end{algorithm}

Issues of the algorithm:
\begin{enumerate}
    \item The above algorithm cannot achieve constant communication, because the optimal arm in UCB algorithm is pulled \(O(T)\) times and, with \alg, is communicated \(O(\log T)\) times.
    \item The pulling times of an arm is different among agents, while \alg is only proved for balanced exploration. However, if I use the global UCB index technique to force a balanced arm exploration with reward mean \(\hat{\mu}_{\texttt{com}}(i)\), there is no guarantee that this common mean is a good reward mean estimate. Is it possible to design an unbalanced \alg algorithm? \begin{itemize}
              \item \textbf{ToDo} let's start from periodic \alg design.
          \end{itemize}
\end{enumerate}

Define \(\Theta^j \coloneqq \sum_{j'\in\mathcal{M}} {\theta_{j'}}/{\Theta^j}\) as the total pulling ratio base on the pulling times of agent \(j\).

\begin{equation}\label{eq:est-auxiliary-periodic}
    \hat{\mu}_{\texttt{aux},t}^j(i)=\frac{1}{\Theta^j n_t^j(i)}\sum_{j'=1}^M \left(X_{\tau(t)}^{j'}(i)+X_t^j(i)-X_{\tau(t)}^j(i)\right)
\end{equation}

\begin{equation}\label{eq:est-periodic}
    \hat{\mu}_{t}^j(i)=\frac{1}{\Theta^j n_{\tau(t)}^j(i)+n_t^j(i)-n_{\tau(t)}^j(i)}\left(\sum_{j'=1}^M X_{\tau(t)}^{j'}(i)+X_t^j(i)-X_{\tau(t)}^j(i)\right)
\end{equation}


\begin{algorithm}[t]
    \caption{\alg with periodic arrivals for agent \(j\)}
    \label{alg:doe-periodic}
    \begin{algorithmic}[1]
        %		\Require $t=1,2,\ldots,T$
        \State \textbf{Parameters:} $\beta>1$; $\ei_n, n=1,2,\dots$, action rates \(\{\theta_1,\dots,\theta_M\}\)
        \State \textbf{Initialization:} $\hat{\mu}_{\texttt{com}}(i), n_t^j(i) \leftarrow 0$, $\hat{\mu}^j_{\texttt{aux},t}(i),\hat{\mu}_t^j(i), \ei_{\tau(t)}^j(i)\gets \infty$, for all $i$, and $G_t^j(i)\leftarrow \alpha \ci(\Theta^j n_t^j(i),\delta)$, $n=1,2,\ldots$
        \For{each round $t$ when the agent gets a new sample}
        \State $n(i)\leftarrow n(i)+1$
        \State Update $X^j(i)$ with the new sample
        %		\State Update the upper and lower confidence bounds as follows:
        %		\begin{equation*}
        %			u(I^j_t)\leftarrow \hat{\mu}(I^j_t) + \sqrt{\frac{\alpha \log \delta_t^{-1}}{2\hat{n}(I^j_t)}},~b(I^j_t)\leftarrow \hat{\mu}(I^j_t) - \sqrt{\frac{\alpha \log \delta_t^{-1}}{2\hat{n}(I^j_t)}}
        %		\end{equation*}
        \If {$\beta G_t^j(i)\leq\ei_{\tau(t)}^j(i)$}\label{line:ratio-condition-periodic}
        \State \(\tau(t) \gets t\) and $\ei_{\tau(t)}^j(i)\leftarrow G_t^j(i)$
        \label{line:update-G-last-periodic}

        \If {$|\hat{\mu}_{\texttt{aux},t}^j(i)-\hat{\mu}_{\texttt{com}}(i)|>G_t^j(i)$}\label{line:deviation-condition-periodic}
        \State{\texttt{//Communicate to synchronize the estimates}}
        \State{--- Collect $X_t^{j'}(i)$ from other agents \(j'\neq j\) and calculate the new $\hat{\mu}_{\texttt{com}}(i)$}
        \State --- Broadcast the new $\hat{\mu}_{\texttt{com}}(i)$ to other agents \(j'\neq j\)
        \State --- $X_{\tau(t)}^{j'}(i)\leftarrow X_t^{j'}(i)$ for all $j'\in \mathcal{M}$
        \EndIf
        \EndIf
        \State Update $n_{t+1}^j(i), \hat{\mu}_{t+1}^j(i)$, and $\hat{\mu}_{\texttt{aux},t+1}^j(i)$
        \EndFor
    \end{algorithmic}
\end{algorithm}

\begin{lemma}\label{lem:ub-periodic} Assume $M$ agents independently sample an arm with an i.i.d. reward process with unknown mean $\mu(i)$, and $n_t^j(i)$ is the available samples for each agent \(j\in\mathcal{M}\) up to time slot $t$. With $\beta >1$ and $\ei_t^j(i)= \alpha \ci(\Theta^j n_t^j(i),\delta)$, we have for any $t$, with probability $1-\delta$,
    \begin{equation*}
        |\hat{\mu}_t^j(i)-\mu(i)|\leq (2\alpha\beta+\beta)\ci\left(\Theta^j n_t^j(i),\delta\right).
    \end{equation*}
\end{lemma}

\begin{proof}[Proof of Lemma~\ref{lem:ub-periodic}]

    We prove the lemma by analyzing the following two cases.
    Let \(s\) denote the last detection point, i.e., the last time slot (before \(t\)) that the condition in Line~\ref{line:ratio-condition-periodic} of Algorithm~\ref{alg:doe-periodic} holds.

    Case (1): the agent communicated at the last detection point $s$. In this case, the estimate $\hat{\mu}_{t}^j(i)$ is obtained by averaging $\Theta^jn_s^j(i)+n_t^j(i)-n_s^j(i)$ samples. Hence, the following equation holds with probability $1-\delta$.
    \begin{equation*}
        \begin{split}
            \abs{\hat{\mu}_{t}^j(i)-\mu(i)}&\leq \ci_{[0,1]}\left(\Theta^jn_s^j(i)+n_t^j(i)-n_s^j(i),\delta\right) \\
            &\overset{(a)}\leq  \ci_{[0,1]}\left(\Theta^jn_s^j(i),\delta\right)\\
            &\overset{(b)}= G_{\text{last}}(i)\\
            &\overset{(c)}\leq  \beta \ci_{[0,1]}\left(\Theta^jn_t^j(i),\delta\right),
        \end{split}
    \end{equation*}
    where inequality (a) is due to that the width of confidence interval increases with smaller number of samples,
    inequality (b) is due to that the condition in Line~\ref{line:ratio-condition-periodic} holds at time slot \(s\) and Line~\ref{line:update-G-last-periodic} is thus executed,
    and inequality (c) is because that the condition in Line~\ref{line:ratio-condition-periodic} is false at time slot \(t\).

    In this case, the result in Lemma~\ref{lem:ub-periodic} holds.


    Case (2): there is no communication at $s$.
    Let $A$ be the sum of samples obtained by agent $j$ if communication \emph{happened} at $s$.
    We have
    \begin{equation*}
        \begin{split}
            &\abs*{
                \left(\Theta^jn_s^j(i)+n_t^j(i)-n_s^j(i)\right)\hat{\mu}_{t}^j(i)
                -A
            } \\
            =&\left|\left(\Theta^jn_s^j(i)\hat{\mu}_{\texttt{aux},s}^j(i) + \left(X_t^j(i)-X_{s}^j(i)\right)\right)
            -\left(\sum_{j'=1}^M X_s^{j'}(i) + \left(X_t^j(i)-X_s^j(i)\right)\right) \right| \\
            =&\left|\Theta^jn_s^j(i)\hat{\mu}_{\texttt{aux},s}^j(i)-\sum_{j'=1}^M X_s^{j'}(i)\right|.
        \end{split}
    \end{equation*}

    The above equation is based on the fact that agent always has the local samples after $s$ even if there is no communication at $s$.

    Hence, dividing both hand sides by \((\Theta^jn_s^j(i)+n_t^j(i)-n_s^j(i))\) leads to
    \begin{equation*}
        \begin{split}
            \left|\hat{\mu}_{t}^j(i)-\frac{A}{\Theta^jn_s^j(i)+n_t^j(i)-n_s^j(i)}\right|
            &=\frac{1}{\Theta^jn_s^j(i)+n_t^j(i)-n_s^j(i)}\left|\Theta^jn_s^j(i)\hat{\mu}_{\texttt{aux},s}^j(i)-\sum_{j'=1}^M X_s^{j'}(i)\right|\\
            &=\frac{\Theta^jn_s^j(i)}{\Theta^jn_s^j(i)+n_t^j(i)-n_s^j(i)}\abs*{\hat{\mu}_{\texttt{aux},s}^j(i)-\frac{1}{\Theta^jn_s^j(i)}\sum_{j'=1}^M X_s^{j'}(i)}\\
            &\leq   \left|\hat{\mu}_{\texttt{aux},s}^j(i)-\frac{1}{\Theta^jn_s^j(i)}\sum_{j'=1}^M X_s^{j'}(i)\right|   \\
            &\overset{\textcolor{red}{\bf (a) ?}}\leq  2\alpha \ci_{[0,1]}(\Theta^jn_s^j(i),\delta)\\
            &\overset{(b)}= 2\alpha G_{\text{last}}(i)\\
            &\overset{(c)}\leq 2\alpha\beta \ci_{[0,1]}(\Theta^jn_t^j(i),\delta),
        \end{split}
    \end{equation*}
    where inequality (a) is because the condition in Line~\ref{line:deviation-condition-periodic} in Algorithm~\ref{alg:doe-periodic} does not hold at time slot \(s\) (since the condition in Line~\ref{line:ratio-condition-periodic} holds but there is no communication at \(s\)):
    \todo{This is a not resolved issue.}
    In this case, $ \left|\hat{\mu}_{\texttt{aux},s}^j(i)-\hat{\mu}_{\texttt{aux},s}^{j'}(i)\right|\leq G_t^j(i) + G^{j'}(n_t^{j'}(i)) =   2\alpha \ci_{[0,1]}(\Theta^jn_s^j(i),\delta)$ for any agents $j$ (one can fix \(j\)) `and $j'$. Also, $\frac{1}{\Theta^jn_s^j(i)}\sum_{j'=1}^M X_s^{j'}(i)$ averages all samples up to $s$, and hence its value lies between $\min_{j'}\hat{\mu}_{\texttt{aux},s}^{j'}(i)$ and $\max_{j'}\hat{\mu}_{\texttt{aux},s}^{j'}(i)$, which weight partial local samples with a factor $M$ to replace missing ones. Combining the two facts, we prove inequality (a).
    Inequality (b) is due to that the condition in Line~\ref{line:ratio-condition-periodic} holds at time slot \(s\) and Line~\ref{line:update-G-last-periodic} is thus executed,
    and inequality (c) is because that the condition in Line~\ref{line:ratio-condition-periodic} is false at time slot \(t\).

    Since $A$ contains the same set of samples as the \(\hat{\mu}_{t}^j(i)\) in Case (1), the following equation also holds with probability $1-\delta$:
    \begin{equation*}
        \left|\frac{A}{\Theta^jn_s^j(i)+n_t^j(i)-n_s^j(i)}-\mu(i)\right|\leq\beta \ci_{[0,1]}\left(\Theta^jn_t^j(i),\delta\right).
    \end{equation*}

    Combining the above two equations yields
    \begin{equation*}
        \left|\hat{\mu}_{t}^j(i)-\mu(i)\right|\leq(2\alpha+1) \beta\ci_{[0,1]}(Mn_t(i),\delta), ~\text{with ~probability}~1-\delta.
    \end{equation*}

    As a result, we prove the  Lemma~\ref{lem:ub-periodic}.
\end{proof}
